Dual Learning for Semi-Supervised Natural Language Understanding

Natural language understanding (NLU) converts sentences into structured semantic forms. The paucity of annotated training samples is still a fundamental challenge of NLU. To solve this data sparsity problem, previous work based on semi-supervised learning mainly focuses on exploiting unlabeled sentences. In this work, we introduce a dual task of NLU, semantic-to-sentence generation (SSG), and propose a new framework for semi-supervised NLU with the corresponding dual model. The framework is composed of dual pseudo-labeling and dual learning method, which enables an NLU model to make full use of data (labeled and unlabeled) through a closed-loop of the primal and dual tasks. By incorporating the dual task, the framework can exploit pure semantic forms as well as unlabeled sentences, and further improve the NLU and SSG models iteratively in the closed-loop. The proposed approaches are evaluated on two public datasets (ATIS and SNIPS). Experiments in the semi-supervised setting show that our methods can outperform various baselines significantly, and extensive ablation studies are conducted to verify the effectiveness of our framework. Finally, our method can also achieve the state-of-the-art performance on the two datasets in the supervised setting. Our code is available at \url{https://github.com/rhythmcao/slu-dual-learning.git}.

==> tables/ablation_study_SSG_old.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet3'
\begin{table*}[t]
  \caption{Ablation studies of the SSG model.}
  \label{tab:ablation_of_SSG_old}%
  \centering{
    \begin{tabular}{l||cc|cc|cc|cc}
    \hline
    \multirow{3}*{\textbf{Method}} & \multicolumn{4}{c|}{\textbf{ATIS}} & \multicolumn{4}{c}{\textbf{SNIPS}} \\
    \cline{2-9}
    & \multicolumn{2}{c|}{\text{NLU}} & \multicolumn{2}{c|}{\text{SSG}} & \multicolumn{2}{c|}{\text{NLU}} & \multicolumn{2}{c}{\text{SSG}} \\
    \cline{2-9}
    & Slot $\text{F}_1$ & Intent Acc & BLEU & Slot Acc &  Slot $\text{F}_1$ & Intent Acc & BLEU & Slot Acc \\
    \hline \hline
    sup & 82.92 & 89.03 & 33.53 & 79.17 & 87.89 & 97.86 & 29.84 & 94.85 \\
    \hline
    dual PL + dual learning & \textbf{89.58} & \textbf{90.48} & 36.62 & \textbf{88.55} & \textbf{94.00} & 98.29 & \textbf{36.61} & 99.43 \\
    \quad(-) w/o feeding intent & 89.42 & 89.47 & 35.77 & 88.34 & 93.73 & 97.71 & 36.07 & \textbf{99.62}  \\
    \quad(-) w/o copy mechanism & 87.52 & 89.92 & 36.54 & 87.91 & 93.58 & \textbf{98.43} & 34.52 & 98.63/99.96  \\
    \quad(-) w/o SC-LSTM & 89.27 & 89.81  & \textcolor{red}{\textbf{36.92}} & 86.98 & 93.74 & 97.86 & 34.10 & 98.87 \\
    \quad(-) w/o global BLSTM & 88.17 & 89.92 & 33.62 & 86.33 & 92.90 & 97.71 & 27.35 & 97.52  \\
    \hline
    \end{tabular}%
  }
\end{table*}%



==> tables/main_results_old.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet3'
\begin{table*}[t]
  \caption{Slot $\text{F}_1$ scores and intent accuracies of different methods on ATIS and SNIPS datasets. We randomly select \{5,10,20,30,50\}\% of the training set as labeled data, and leave the rest as unpaired sentences and semantic forms to simulate unlabeled data. The results in bold black are the best slot F$_1$ scores and intent accuracies.}
  \label{tab:main_results_on_atis_snips}%
  \centering{
    \begin{tabular}{l|l|cccccc|cccccc}
    \hline
    \multicolumn{2}{l|}{\multirow{2}*{\diagbox{\textbf{Method}}{\textbf{\ \ \ \ Slot $\text{F}_1$} (\%)}}} & \multicolumn{6}{c|}{\textbf{ATIS}} & \multicolumn{6}{c}{\textbf{SNIPS}} \\
    \cline{3-14}
    \multicolumn{2}{c|}{} & 5\% & 10\% & 20\% & 30\% & 50\% & 100\% & 5\% & 10\% & 20\% & 30\% & 50\% & 100\% \\
    \hline
    \multirow{1}*{supervised} & \textbf{BLSTM-focus} (backbone) & 82.92 & 89.48 & 92.66 & 93.54 & 95.45 & 95.79 & 87.89 & 91.23 & 93.54 & 94.45 & 94.92 & \textbf{96.44}$^\ddagger$ \\
    %& BLSTM-softmax & 83.64 & 89.26 & 92.28 & 93.59 & 94.38 & 95.50 & 85.61 & 89.78 & 91.83 & 93.45 & 94.54 & 94.96 \\
    %& BLSTM-crf & 83.94 & 90.38 & 92.60 & 94.17 & 95.23 & 95.62 & 87.25 & 90.83 & 93.19 & 94.35 & 94.74 & 96.34 \\
    \hline
    \multirow{3}*{\begin{tabular}[c]{@{}l@{}}semi-\\ supervised\end{tabular}} & \ \ + sentence auto-encoder & 83.16 & 89.65 & 92.74 & 94.52 & 95.36 & 95.80 & 87.83 & 89.81 & 92.55 & 93.47 & 93.34 & 95.72 \\
    & \ \ + pseudo-labeling (PL) & 84.75 & 90.08 & 94.07 & 94.91 & 95.52 & 95.75 & 90.67 & 91.89 & 93.89 & 94.29 & 95.06 & 96.00 \\
    & \ \ + template synthesis & 86.10 & 90.62 & 94.35 & 94.94 & 95.27 & - & 90.40 & 92.94 & 93.94 & 94.22 & 94.37 & - \\
    \hline
    \multirow{3}*{\begin{tabular}[c]{@{}l@{}}+ dual task\\(ours)\end{tabular}} & \ \ + dual PL & \textbf{89.58}$^\ddagger$ & 93.49$^\ddagger$ &  94.88 & \textbf{95.90}$^\ddagger$ & 96.02$^\ddagger$ & 95.82 & 93.86 & 94.46 & \textbf{95.53} & 95.23 & 95.29$^\ddagger$ & 96.22$^\ddagger$ \\
    & \ \ + dual learning &  88.92 & 93.40$^\ddagger$ & 95.09$^\ddagger$ & 95.50 & 95.70 & 96.00 & 93.85 & 94.18 & 95.31 & 95.08 & \textbf{95.45}$^\ddagger$ & 95.86 \\
    & \ \ + dual PL + dual learning &  \textbf{89.58}$^\ddagger$ & \textbf{93.53}$^\ddagger$ & \textbf{95.37}$^\ddagger$ & 95.85$^\ddagger$ & \textbf{96.14}$^\ddagger$ & \textbf{96.37}$^\ddagger$ & \textbf{94.00} & \textbf{94.51} & 95.22 & \textbf{95.34} & 95.25$^\ddagger$ & 96.11$^\ddagger$ \\
    \hline
        \hline
    \multicolumn{2}{l|}{\multirow{2}*{\diagbox{\textbf{Method}}{\textbf{Intent Acc} (\%)}}} & \multicolumn{6}{c|}{\textbf{ATIS}} & \multicolumn{6}{c}{\textbf{SNIPS}} \\
    \cline{3-14}
    \multicolumn{2}{c|}{} & 5\% & 10\% & 20\% & 30\% & 50\% & 100\% & 5\% & 10\% & 20\% & 30\% & 50\% & 100\% \\
    \hline
    \multirow{1}*{supervised} & \textbf{BLSTM-focus} (backbone) & 89.03 & 92.61 & 94.40 & 94.85 & \textbf{98.54} & 98.43 & 97.86 & 98.14 & 98.00 & 98.29 & 98.71 & \textbf{99.14} \\
    %& BLSTM-softmax & 89.59 & 92.50 & 92.95 & 93.51 & 98.21 & 98.21 & 97.57 & 98.29 & 98.00 & \textbf{98.57} & 98.71 & 98.86 \\
    %& BLSTM-crf & 89.70 & 92.50 & 93.73 & 93.51 & 98.32 & 98.32 & 97.43 & 98.29 & 98.43 & 98.43 & 98.43 & 98.86 \\
    \hline
    \multirow{3}*{\begin{tabular}[c]{@{}l@{}}semi-\\ supervised\end{tabular}} & \ \ + sentence auto-encoder & 88.80 & 92.50 & \textbf{95.30} & 94.62 & 98.32 & 98.32 & 96.86 & 97.86 & 98.14 & 98.00 & 98.71 & 98.86 \\
    & \ \ + pseudo-labeling (PL) & 89.47 & 92.50 & 95.18 & 94.85 & 98.32 & 98.32 & 97.57 & 98.00 & 98.14 & 98.00 & 99.00 & \textbf{99.14} \\
    & \ \ + template synthesis & 90.05 & 92.05 & 94.06 & 94.51 & 98.10 & - & 97.86 & 98.00 & \textbf{98.57} & 98.14 & 98.86 & - \\
    \hline
    \multirow{3}*{\begin{tabular}[c]{@{}l@{}}+ dual task\\(ours)\end{tabular}} & \ \ + dual PL & 90.37 & 93.28 & 94.62 & \textbf{96.08} & 98.43 & \textbf{98.66} & \textbf{98.57} & 98.14 & 98.43 & 98.43 & 98.71 & \textbf{99.14} \\
    & \ \ + dual learning & 89.81 & 93.28 & \textbf{95.30} & 95.86 & \textbf{98.54} & 98.54 & 98.29 & 98.14 & 98.29 & \textbf{98.57} & 98.57 & 98.86 \\
    & \ \ + dual PL + dual learning &  \textbf{90.48} & \textbf{93.51} & 95.18 & 95.30 & \textbf{98.54} & 98.54 & 98.29 & \textbf{98.43} & \textbf{98.57} & 98.14 & \textbf{99.14} & 98.86 \\
    \hline
    \end{tabular}%
  }
\end{table*}%












% Table generated by Excel2LaTeX from sheet 'Sheet3'
\begin{table*}[t]
  \caption{Slot $\text{F}_1$ scores and intent accuracies of different methods on ATIS and SNIPS datasets. We randomly select \{5,10,20,30,50\}\% of the training set as labeled data, and leave the rest as unpaired sentences and semantic forms to simulate unlabeled data.}
  \label{tab:main_results_on_atis_snips}%
  \centering{
    \begin{tabular}{l|l|cccccc|cccccc}
    \hline
    \multicolumn{2}{c|}{\multirow{2}*{\textbf{Method}}} & \multicolumn{6}{c|}{\textbf{ATIS} (Slot $\text{F}_1$)} & \multicolumn{6}{c}{\textbf{SNIPS} (Slot $\text{F}_1$)} \\
    \cline{3-14}
    \multicolumn{2}{c|}{} & 5\% & 10\% & 20\% & 30\% & 50\% & 100\% & 5\% & 10\% & 20\% & 30\% & 50\% & 100\% \\
    \hline
    \multirow{3}*{sup} & BLSTM-softmax & 83.64 & 89.26 & 92.28 & 93.59 & 94.38 & 95.50 & 85.61 & 89.78 & 91.83 & 93.45 & 94.54 & 94.96 \\
    & BLSTM-crf & 83.94 & 90.38 & 92.60 & 94.17 & 95.23 & 95.62 & 87.25 & 90.83 & 93.19 & 94.35 & 94.74 & 96.34 \\
    & \textbf{BLSTM-focus} & 82.92 & 89.48 & 92.66 & 93.54 & 95.45 & 95.79 & 87.89 & 91.23 & 93.54 & 94.45 & 94.92 & \textbf{96.44} \\
    \hline
    \multirow{3}*{\begin{tabular}[c]{@{}l@{}}semi-\\ sup\end{tabular}} & + sentence auto-encoder & 83.16 & 89.65 & 92.74 & 94.52 & 95.36 & 95.80 & 87.83 & 89.81 & 92.55 & 93.47 & 93.34 & 95.72 \\
    & + pseudo-labeling (PL) & 84.75 & 90.08 & 94.07 & 94.91 & 95.52 & 95.75 & 90.84 & 91.89 & 93.89 & 94.29 & 95.06 & 96.00 \\
    & + template synthesis & 86.10 & 90.62 & 94.35 & 94.94 & 95.27 & - & 90.40 & 92.72 & 93.94 & 94.22 & 94.37 & - \\
    \hline
    \multirow{3}*{ours} & + dual PL & \textbf{89.58} & 92.92 &  94.88 & \textbf{95.90} & 96.02 & 95.82 & 93.86 & 94.46 & \textbf{95.53} & 95.23 & 95.29 & 96.22 \\
    & + dual learning &  \textcolor{red}{87.99} & 93.40 & 95.09 & 95.50 & 95.70 & 96.00 & 93.85 & 94.18 & 95.31 & 95.08 & \textbf{95.45} & 95.86 \\
    & + dual PL + dual learning &  \textbf{89.58} & \textbf{93.53} & \textbf{95.37} & 95.85 & \textbf{96.14} & \textbf{96.37} & \textbf{94.00} & \textbf{94.51} & 95.22 & \textbf{95.34} & 95.25 & 96.08 \\
    \hline
        \hline
    \multicolumn{2}{c|}{\multirow{2}*{\textbf{Method}}} & \multicolumn{6}{c|}{\textbf{ATIS} (Intent Acc)} & \multicolumn{6}{c}{\textbf{SNIPS} (Intent Acc)} \\
    \cline{3-14}
    \multicolumn{2}{c|}{} & 5\% & 10\% & 20\% & 30\% & 50\% & 100\% & 5\% & 10\% & 20\% & 30\% & 50\% & 100\% \\
    \hline
    \multirow{3}*{sup} & BLSTM-softmax & 89.59 & 92.50 & 92.95 & 93.51 & 98.21 & 98.21 & 97.57 & 98.29 & 98.00 & \textbf{98.57} & 98.71 & 98.86 \\
    & BLSTM-crf & 89.70 & 92.50 & 93.73 & 93.51 & 98.32 & 98.32 & 97.43 & 98.29 & 98.43 & 98.43 & 98.43 & 98.86 \\
    & \textbf{BLSTM-focus} & 89.03 & 92.61 & 94.40 & 94.85 & \textbf{98.54} & 98.32 & 97.86 & 98.14 & 98.00 & 98.29 & 98.71 & \textbf{99.14} \\
    \hline
    \multirow{2}*{\begin{tabular}[c]{@{}l@{}}semi-\\ sup\end{tabular}} & + sentence auto-encoder & 88.80 & 92.50 & \textbf{95.52} & 94.62 & 98.32 & 98.32 & 96.86 & 97.86 & 98.14 & 98.00 & 98.71 & 98.86 \\
    & + pseudo-labeling (PL) & 89.47 & 92.50 & 95.18 & 94.85 & 98.32 & 98.32 & 98.29 & 98.00 & 98.14 & 98.00 & 99.00 & \textbf{99.14} \\
    & + template synthesis & 90.05 & 92.05 & 94.06 & 94.51 & 98.10 & - & 97.86 & \textbf{99.00} & \textbf{98.57} & 98.14 & 98.86 & - \\
    \hline
    \multirow{3}*{ours} & + dual PL & 90.37 & 93.28 & 94.62 & \textbf{96.08} & 98.43 & \textbf{98.66} & \textbf{98.57} & 98.14 & 98.43 & 98.43 & 98.71 & \textbf{99.14} \\
    & + dual learning & 89.81 & 92.83 & 94.85 & 95.41 & \textbf{98.54} & 98.32 & 98.29 & 98.29 & 98.29 & \textbf{98.57} & 98.57 & 98.86 \\
    & + dual PL + dual learning &  \textbf{90.48} & \textbf{93.51} & 95.18 & 95.30 & \textbf{98.54} & 98.54 & 98.29 & 98.29 & 98.29 & 98.14 & \textbf{99.14} & 98.71 \\
    \hline
    \end{tabular}%
  }
\end{table*}%


